Physics at a future Neutrino Factory and super-beam facility

The conclusions of the Physics Working Group of the international scoping study of a future Neutrino Factory and super-beam facility (the ISS) are presented. The ISS was carried by the international community between NuFact05, (the 7th International Workshop on Neutrino Factories and Superbeams, Laboratori Nazionali di Frascati, Rome, June 21-26, 2005) and NuFact06 (Ivine, California, 24{30 August 2006). The physics case for an extensive experimental programme to understand the properties of the neutrino is presented and the role of high-precision measurements of neutrino oscillations within this programme is discussed in detail. The performance of second generation super-beam experiments, beta-beam facilities, and the Neutrino Factory are evaluated and a quantitative comparison of the discovery potential of the three classes of facility is presented. High-precision studies of the properties of the muon are complementary to the study of neutrino oscillations. The Neutrino Factory has the potential to provide extremely intense muon beams and the physics potential of such beams is discussed in the final section of the report.

==> 02-Standard-Neutrino-Model/02-02-Challenges-for-the-future.tex <==
\subsubsection{Summary: Challenges for the future}

To summarise, the main experimental challenges facing neutrino physics,
{\em without yet assuming the presence of new physics effects
in neutrino oscillations} include the following:
\begin{itemize}
  \item 
    The sign of $\Delta m^2_{31}$: whether the neutrino mass
    ordering is ``normal'' or ``inverted'' has important implications for
    Grand Unification, Flavour Models and Cosmology. 
  \item 
    The question of CP-violation ($\delta$): measurement of 
    the oscillation phase represents 
    the Holy Grail of neutrino physics, since it would signal
    CP violation in the lepton sector, which would also have profound
    implications for Grand Unification, Flavour Models and Cosmology. 
  \item 
    High precision measurements of mixing angles: especially
    $\theta_{13}$ which has so far not been measured at all;
    a high precision determination of all the mixing angles 
    to the same level of precision as the quark mixing angles,
    again provides crucial information for Grand Unification and Flavour Models.
\end{itemize}

A Neutrino Factory would provide the best possible
experimental information on these
outstanding challenges currently facing neutrino physics.
The remaining
questions (below) 
could be addressed by a combination of Neutrinoless Double Beta
decay experiments, Tritium end-point experiments and Cosmological
considerations:

\begin{itemize}
  \item 
    Majorana vs Dirac: the question of whether neutrino masses
    are Majorana or Dirac in nature has profound implications 
    for particle physics.
  \item 
    The absolute neutrino mass scale: only mass squared
    differences are relevant for neutrino oscillations, and the
    absolute neutrino mass scale is so far not measured.
\end{itemize}

So far we have been assuming that there is no new physics that
will be observable in neutrino oscillations,
as would be the case for the see-saw mechanism
implemented at a high energy scale.
Even in this minimal case the challenges facing
neutrino physics require new high precision 
experiments to address the challenges discussed
in the previous section.
However it is possible that high precision 
neutrino facilities will reveal qualitatively new
physics effects beyond the minimal see-saw case so far
discussed. Although this is not guaranteed, and to a large
extent such discoveries cannot be anticipated, the discovery
of such new physics in neutrino oscillations would represent
such a monumental discovery that it is worth surveying
some of the possibilities in the following subsection.



==> 04-BSnuM/04-01-Sterile-neutrino/def_temp.tex <==
%-- commands -----------------------------------------------------

\newcommand{\eVq}{\text{eV}^2}
\newcommand{\CL}   {C.L.}
\newcommand{\dof}  {d.o.f.}
\newcommand{\Sol}  {\textsc{sol}}
\newcommand{\SlKm} {\textsc{sol+kam}}
\newcommand{\Atm}  {\textsc{atm}}
\newcommand{\KtK}  {\textsc{k2k}}
\newcommand{\Chooz}{\textsc{chooz}}
\newcommand{\Dms}  {\Delta m^2_{21}}
\newcommand{\Dma}  {\Delta m^2_{31}}
\newcommand{\Lsnd} {\textsc{lsnd}}
\newcommand{\Dml}  {\Delta m^2_\Lsnd}
\newcommand{\Sbl}  {\textsc{sbl}}
\newcommand{\Nev}  {\textsc{nev}}



==> MakeClean <==
#!/bin/csh -f

rm -f *.log
rm -f *.out
rm -f *.toc
rm -f *.aux
rm -f *.dvi
rm -f *.blg

find . -name '#*#' -print -exec rm '{}' \;
find . -name '*~' -print -exec rm '{}' \;

